Cohomology of complete unordered flag manifolds

We consider quotients of complete flag manifolds in Cn and Rn by an action of the symmetric group on n objects. We compute their cohomology with field coefficients of any characteristic. Specifically, we show that these topological spaces exhibit homological stability and we provide a closed-form description of their stable cohomology rings. We also describe a simple algorithmic procedure to determine their unstable cohomology additively.

==> Section7.tex <==
% !TEX root = Unordered flag varieties.tex

\section{Application to Auerbach bases and the Pełczyński conjecture}

%%% Local Variables:
%%% TeX-master: "Unordered flag varieties.tex"
%%% End:
